Very Large Language Model as a Unified Methodology of Text Mining

Text data mining is the process of deriving essential information from language text. Typical text mining tasks include text categorization, text clustering, topic modeling, information extraction, and text summarization. Various data sets are collected and various algorithms are designed for the different types of tasks. In this paper, I present a blue sky idea that very large language model (VLLM) will become an effective unified methodology of text mining. I discuss at least three advantages of this new methodology against conventional methods. Finally I discuss the challenges in the design and development of VLLM techniques for text mining.

==> bib.tex <==
\bibitem{aggarwal2012mining}
C.~C. Aggarwal and C. Zhai, {\em Mining text data}. Springer, Boston, MA. (2012).

\bibitem{aggarwal2015mining}
C.~C. Aggarwal, {\em Mining text data}, Data Mining. Springer, Cham. (2015).

\bibitem{zong2021text}
C. Zong, R. Xia, and J. Zhang, {\em Text data mining}, Singapore: Springer. (2021).



% \bibitem{BANKSMITH}
% R.~E. Bank and R.~K. Smith, {\em General sparse elimination requires no
%   permanent integer storage}, SIAM J. Sci. Stat. Comput., 8 (1987),
%   pp.~574--584.

% \bibitem{EISENSTAT}
% S.~C. Eisenstat, M.~C. Gursky, M.~Schultz, and A.~Sherman, {\em
%   Algorithms and data structures for sparse symmetric gaussian elimination},
%   SIAM J. Sci. Stat. Comput., 2 (1982), pp.~225--237.

% \bibitem{GEORGELIU}
% A.~George and J.~Liu, {\em Computer Solution of Large Sparse Positive
%   Definite Systems}, Prentice Hall, Englewood Cliffs, NJ, 1981.

% \bibitem{LAW}
% K.~H. Law and S.~J. Fenves, {\em A node addition model for symbolic
%   factorization}, ACM TOMS, 12 (1986), pp.~37--50.

% \bibitem{LIU}
% J.~W.~H. Liu, {\em A compact row storage scheme for cholesky factors
%   using elimination trees}, ACM TOMS, 12 (1986), pp.~127--148.

% \bibitem{LIU2}
% \sameauthor , {\em The role of
%   elimination trees in sparse factorization}, Tech. Report CS-87-12,Department
%   of Computer Science, York University, Ontario, Canada, 1987.

% \bibitem{ROSE72}
% D.~J. Rose, {\em A graph theoretic study of the numeric solution of
%   sparse positive definite systems}, in Graph Theory and Computing, Academic  Press, New
% York, 1972.

% \bibitem{ROSE76}
% D.~J. Rose, R.~E. Tarjan, and G.~S. Lueker, {\em Algorithmic aspects of
%   vertex elimination on graphs}, SIAM J. Comput., 5 (1976), pp.~226--283.

% \bibitem{ROSEWHITTEN}
% D.~J. Rose and G.~F. Whitten, {\em A recursive analysis of disection
%   strategies}, in Sparse Matrix Computations, Academic Press, New York, 1976.

% \bibitem{SCHREIBER}
% R.~Schrieber, {\em A new implementation of sparse gaussian elimination},
%   ACM TOMS, 8 (1982), pp.~256--276.

